UncertainSAM: Fast and Efficient Uncertainty Quantification of the Segment Anything Model

The introduction of the Segment Anything Model (SAM) has paved the way for numerous semantic segmentation applications. For several tasks, quantifying the uncertainty of SAM is of particular interest. However, the ambiguous nature of the class-agnostic foundation model SAM challenges current uncertainty quantification (UQ) approaches. This paper presents a theoretically motivated uncertainty quantification model based on a Bayesian entropy formulation jointly respecting aleatoric, epistemic, and the newly introduced task uncertainty. We use this formulation to train USAM, a lightweight post-hoc UQ method. Our model traces the root of uncertainty back to under-parameterised models, insufficient prompts or image ambiguities. Our proposed deterministic USAM demonstrates superior predictive capabilities on the SA-V, MOSE, ADE20k, DAVIS, and COCO datasets, offering a computationally cheap and easy-to-use UQ alternative that can support user-prompting, enhance semi-supervised pipelines, or balance the tradeoff between accuracy and cost efficiency.

==> figures/uncertainty_estimation.tex <==
\begin{figure*}[ht]
\centering

\begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/uncertainty_estimation/scores_segmentation-tiny_ade20k_ade20k.pdf}
         \caption{Evaluated on ADE20k}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/uncertainty_estimation/scores_segmentation-tiny_ade20k_coco.pdf}
         \caption{Evaluated on COCO}
     \end{subfigure}

\caption{Uncertainty Estimation in Segmentation: Trained on ADE20k (Model Tiny).} 
\label{fig:uncertainty_estimation_ade20k}
\end{figure*}

==> rebuttal.tex <==
#################### R1: nnaG ########################################
Summary:

The paper introduces UncertainSAM (USAM), a method for uncertainty quantification (UQ) in the Segment Anything Model (SAM). By decomposing uncertainty into epistemic (model), aleatoric (prompt/task), and task ambiguity components, USAM employs a Bayesian entropy framework and lightweight MLPs to estimate uncertainty efficiently. Experimental results across multiple datasets demonstrate USAM's superiority over SAM's inherent confidence score and standard UQ baselines, offering a practical solution for applications requiring reliability and efficiency.
Claims And Evidence: good
Methods And Evaluation Criteria: good
Theoretical Claims: good
Experimental Designs Or Analyses: good
Supplementary Material: good
Relation To Broader Scientific Literature: Please see weakness
Essential References Not Discussed: None
Other Strengths And Weaknesses:
Strengths:
    1. It introduces a novel decomposition of uncertainty into epistemic, prompt, and task sources, addressing SAM's unique class-agnostic nature. This provides a nuanced framework for understanding SAM's limitations. WDSI effectively addresses the challenge of progressive occlusion, where parts of objects become invisible due to overlapping or changes in camera viewpoint. By leveraging hypergraph representations and the WSW metric, the framework ensures reliable tracking and segmentation even in occlusion-heavy scenes.
    2. USAM’s lightweight MLPs achieve state-of-the-art performance while avoiding the computational overhead of Bayesian methods. Extensive experiments on five datasets (DAVIS, ADE20k, MOSE, COCO, SA-V) validate USAM’s effectiveness in tasks like model selection, prompt refinement, and task supervision.
Weaknesses
    1. While USAM outperforms SAM’s confidence score and entropy-based methods, it does not compare against recent SAM-specific UQ approaches (e.g., prompt-augmented methods), leaving its relative novelty unclear. And, though USAM is claimed to be efficient, no runtime or memory benchmarks are provided to quantify gains over Bayesian sampling or other UQ methods. This information would help researchers understand the practical feasibility of implementing USAM.
    2. The MLP architecture and SMAC3 optimization setup are underdescribed. The author should provide more structural diagrams to clarify.
    3. As a lightweight method, the authors should add parameter and speed comparison.
Other Comments Or Suggestions: none
Questions For Authors: please see weakness
Overall Recommendation: 2: Weak reject (i.e., leaning towards reject, but could also be accepted)


-----> TODOs: 
0. Fragen, wie das mit der "WDSI effectively addresses" gemeint ist? It offensichtlich von einem anderen Review da rein gepackt. Sollte man das dem AC auch sagen?
1.1. Anmerkung zu R3, da dieser auch andere Methoden sehen will.
1.2. und 3. Können wir ausrechnen oder auch messen: Sollte sehr sehr gering sein --> Add to repository
2. Informationen zum MLP und SMAC3 geben

-----> REBUTTAL

Thanks to the reviewer for the detailed feedback and comprehensible remarks that will help enhance the paper. Our responses to the mentioned weaknesses and questions are as follows:

1. We only partially agree with the statement that we do not compare to SAM-specific UQ. For example, our Prompt UQ is closely related to Deng et al. (2023, see main paper for reference). Furthermore, SAM-specific UQ is usually application-specific and not readily translatable to our holistic view of UQ. However, this weakness needs to be addressed with a modification of the paper, which is further elaborated in our response to reviewer 3EoJ, who identified a similar concern.

2. We agree that the architecture is underdescribed. It is motivated by SAM's original MLP design for predicting the SamScore. We differ only in the input dimension and hidden state (from 256 to 512) because we employ and concatenate both tokens. We suggest the following modifications to clarify this in the paper:

Line 237: "The simple design of the MLPs aligns with the architecture of SAM’s inherent MLP for predicting the SamScore, as described in the Appendix of Kirillov et al. (2023). They have three layers and a sigmoid activation, but we use 512 input dimensions and hidden states due to the concatenated input tokens. The architecture is visualized in Figure XX."

Additionally, we will include a figure presenting an MLP with the input tokens.

Regarding SMAC3: Due to space limitations, we presented the upper and lower hyperparameter bounds optimized using SMAC3 in ll. 247–252 (right column). We suggest adding a more detailed description and presenting the per-iteration results in tabular form. Since the optimization is not the primary focus of the paper, we would include this in the Appendix and refer to it in line 252. The SMAC3 results will provide greater transparency regarding the robustness of the proposed method.

3. Our proposed MLPs are very small compared to the entire SAM model and require only a single forward pass, unlike MC-based methods. However, as mentioned by the reviewer, an explicit performance comparison should be included in the final version of the paper to demonstrate the impact of our method on efficiency. To address this, we designed hardware-dependent runtime experiments and added them to our anonymous code repository at https://anonymous.4open.science/r/UncertainSAM-C5BF/scripts/speed_test.ipynb for reproducibility.

To illustrate the practical efficiency impact, we conducted tests on a small consumer GPU (GeForce RTX 3050) with the large SAM model, using the hyperparameters described in the paper. Notably, we performed the test with all nine (!) MLPs presented in our paper. Thus, the efficiency of our method could be increased by up to a factor of nine if only specific MLPs are necessary for a given application. We thank the reviewer for this suggestion and propose adding the following results (extended to all models) in an additional table in the final paper.



Large model:
RUNTIME:
SAM2: 0.43796 s per iteration
SAM2 with Entropy: 0.45278 s per iteration
SAM2 with 5 MC image augmentations: 2.18681 s per iteration
SAM2 with 8 MC prompt augmentations: 0.50030 s per iteration
SAM2 with all 9 (!) MLPs proposed in USAM: 0.44144 s per iteration
PARAMETER
SAM2: 224,430,130 parameter
SAM2 with Entropy: 224,430,130 parameter
SAM2 with 5 MC image augmentations: 224,430,130 parameter
SAM2 with 8 MC prompt augmentations: 224,430,130 parameter
SAM2 with all 9 (!) MLPs proposed in USAM: (224,430,130 + 9 x 525,825) parameter

Base+ model:
RUNTIME:
SAM2: 0.20538 s per iteration
SAM2 with Entropy: 0.23294 s per iteration
SAM2 with 5 MC image augmentations: 1.02753 s per iteration
SAM2 with 8 MC prompt augmentations: 0.28902 s per iteration
SAM2 with all 9 (!) MLPs proposed in USAM: 0.20966 s per iteration
PARAMETER
SAM2: 80,833,666 parameter
SAM2 with Entropy: 80,833,666 parameter
SAM2 with 5 MC image augmentations: 80,833,666 parameter
SAM2 with 8 MC prompt augmentations: 80,833,666 parameter
SAM2 with all 9 (!) MLPs proposed in USAM: (80,833,666 + 9 x 525,825) parameter

Small model:
RUNTIME:
SAM2: 0.13444 s per iteration
SAM2 with Entropy: 0.15716 s per iteration
SAM2 with 5 MC image augmentations: 0.68734 s per iteration
SAM2 with 8 MC prompt augmentations: 0.23210 s per iteration
SAM2 with all 9 (!) MLPs proposed in USAM: 0.14160 s per iteration
PARAMETER
SAM2: 46,043,842 parameter
SAM2 with Entropy: 46,043,842 parameter
SAM2 with 5 MC image augmentations: 46,043,842 parameter
SAM2 with 8 MC prompt augmentations: 46,043,842 parameter
SAM2 with all 9 (!) MLPs proposed in USAM: (46,043,842 + 9 x 525,825) parameter

Tiny model:
RUNTIME:
SAM2: 0.12166 s per iteration
SAM2 with Entropy: 0.14876 s per iteration
SAM2 with 5 MC image augmentations: 0.58362 s per iteration
SAM2 with 8 MC prompt augmentations: 0.19736 s per iteration
SAM2 with all 9 (!) MLPs proposed in USAM: 0.13899 s per iteration
PARAMETER
SAM2: 38,945,986 parameter
SAM2 with Entropy: 38,945,986 parameter
SAM2 with 5 MC image augmentations: 38,945,986 parameter
SAM2 with 8 MC prompt augmentations: 38,945,986 parameter
SAM2 with all 9 (!) MLPs proposed in USAM: (38,945,986 + 9 x 525,825) parameter



(Vielleicht den folgenden Punkt weg lassen, weil es so wie sehr unsympathisches Klugscheissern klingt?) 
Finally, we wanted to ask if the two sentence about WDSI is a mistake? 


#################### R2: 6x8E ########################################
Summary:

This paper makes a series of efforts to enable uncertainty quantification for SAM. To achieve this, the authors first adopt Monte Carlo sampling to estimate the predictive, epistemic model, aleatoric prompt, and aleatoric task uncertainty. Then, to release the computation burden of the sampling process during testing, the authors concatenate SAMs 256-dimensional mask and IoU tokens and feed them into MLPs that are trained to predict uncertainty.
Claims And Evidence: The claims are well-supported by the experiments.
Methods And Evaluation Criteria: The proposed method is reasonable.
Theoretical Claims: There are no new theoretical proofs.
Experimental Designs Or Analyses: The experimental designs are reasonable with no major issues. One minor issue is the lack of details on how to combine SAM and SAM2 for the evaluation.
Supplementary Material: I review visualization results for samples with uncertainty estimations.
Relation To Broader Scientific Literature: This work extends the existing Uncertainty Quantification into SAMs.
Essential References Not Discussed: No
Other Strengths And Weaknesses:

Strengths

    1. Uncertainty quantification is important for segmentation tasks.
    2. The decomposition of aleatoric uncertainty into prompt and task uncertainty is reasonable.
    3. The proposed method is easy to follow.

Weaknesses

    1. Lacks the analysis of why the mask and IoU tokens can reflect the uncertainty. Since the uncertainty depends on the ground truth mask, the mask and IoU tokens can not reflect uncertainty entirely.
    2. Why choose MLPs and how to confirm their specific parameters e.g., 3 Layers with 512 hidden states and a Sigmoid activation.

Other Comments Or Suggestions: No other comments.
Questions For Authors:

Since the uncertainty depends on the ground truth mask, the mask and IoU tokens can not reflect uncertainty entirely. Thus, it remains questionable that the usage of only the mask and IoU tokens can reflect the uncertainty.
Code Of Conduct: Affirmed.
Overall Recommendation: 3: Weak accept (i.e., leaning towards accept, but could also be rejected)

-----> TODOs: 
1. Differenz zwischen SAM1 and SAM2 erklären (genau wie bei R3)
2. Ob Uncertainty in Tokens codiert ist wird angezweifelt. Vielleicht Vergleich zu anderen SDN Methoden wie z.B. SamScore geben? Ggf. eine Ablation mit nur einem der beiden Token machen?
3. SIMILAR TO SAM! MLP Parameterisierung beschreiben? Vielleicht auch sagen, dass es nicht so relevant ist und wir uns an das Design vom SamScore angelehnt haben?


----> REBUTTAL:

We want to thank the reviewer for highlighting weaknesses and asking questions that are valuable for enhancing our paper in terms of readability and evaluation. Before addressing the questions, we need to clarify an issue that affects this review as well as reviewer 3EoJ.

After carefully re-reading the paper with temporal distance, we acknowledge that our description of the employment of SAM2 is misleading and needs to be improved.

First, line 254 (right column), "We combine the evaluation of SAM and SAM2," is misleading because we do not combine the models during evaluation. Rather, we combine the datasets evaluated in the corresponding papers. We do this to provide a broader overview that also includes the latest data publication from SAM2.

Second, line 242 (right column), "We use the pretrained SAM2," suggests that we employ SAM2, which is designed for segmenting temporally consistent masks in videos. In reality, while we use the pretrained SAM2 model, we only use its single-image implementation, which is equivalent to SAM and does not include the video extension. We do this because the authors of SAM2 provide more stable code, better interfaces, and slightly better accuracy.

Potentially, our MLPs could be used ad hoc to estimate uncertainty from the refined tokens of SAM2 applied to videos, but that is not evaluated and is beyond the scope of this paper. To prevent misunderstandings for future readers, we propose avoiding the term SAM2 and suggest the following modifications in the camera-ready version:

Replace: "In our experiments, we use the pretrained SAM2 (Ravi et al., 2024)"
With: "In our experiments, we use SAM models pretrained by Ravi et al. (2024)."

Replace: "We combine the evaluation of SAM and SAM2 ..."
With: "Combining the dataset selection of Kirillov et al. and Ravi et al., we ..."

1. Why the mask and IoU tokens can reflect uncertainty

(Un)certainty refers to the likelihood that the prediction is correct. In our case, correctness is measured by the IoU metric, making the expected IoU an ideal proxy for uncertainty. In general, estimating uncertainty does not require ground truth. For example, predictive uncertainty is often described as the variance of the predictive distribution. As seen in Equations 1 and 2, this distribution does not depend on the ground truth. Therefore, the absence of ground truth during inference does not invalidate the expressiveness of our method that uses tokens for uncertainty estimation.

Additionally, the SamScore in SAM (Kirillov et al.) is based on the same principle and also does not have access to ground truth during inference. However, the question of whether and how the mask and IoU tokens reflect uncertainty is an interesting one.

Essentially, the MLPs attempt to map patterns from the object’s latent space (i.e., the tokens) to the expected IoU gap (i.e., uncertainty) based on statistical evidence. The already given effectiveness of the SamScore suggests that such patterns exist in general. To further investigate this question and provide more details for future readers, we conducted an additional ablation study. In this study, we set either the IoU token or the mask token to 0 to remove potentially informative patterns.

We evaluated the predictive capabilities on the COCO dataset using the tiny model across the three tasks described in the submitted paper. The results indicate that both tokens contribute comparably and redundantly to predictive capability, yet they remain accurate as standalone features. The results are:

## Uncertainty Comparison

| Type                 | USAM  | No Mask Token | No IoU Token |
|----------------------|-------|--------------|-------------|
| **Model**           | 63.66 | 61.19        | 62.63       |
| **Prompt**          | 78.30 | 72.08        | 76.42       |
| **Task**           | 94.82 | 86.89        | 91.96       |

We propose to add the findings to the camera ready version.


2. The MLPs' design choice

The reviewer’s remark about our MLP design choice is similar to the comment from reviewer nnaG, indicating that our current explanation lacks clarity. There was no dedicated architecture design process for the UQ estimator. Instead, the architecture is motivated by SAM’s original MLP design for predicting the SamScore. We differ only in the input dimension and hidden states (increasing from 256 to 512) because we employ and concatenate both tokens instead of using just one.

The sigmoid activation function is a reasonable choice since the expected IoU gap ranges between 0 and 1. To improve clarity, we suggest modifying the method description and adding a figure to illustrate the MLP architecture. Please see our response to reviewer nnaG for details on the suggested changes.








#################### R3: 3EoJ ########################################
Summary:

This paper introduces an interesting method to measure the uncertainty of SAM in image segmentation tasks. To achieve this, this paper proposes USAM, an efficient post-hoc method that can quantify the uncertainty of SAM and help users determine whether the model results are reliable, which tunes a lightweight MLP-based estimator. Specifically, the authors design a formula based on Bayesian entropy that can simultaneously consider three levels of uncertainty: model uncertainty (for example, the model is too small, resulting in inaccurate predictions), prompt uncertainty like ambiguous user prompts, and task uncertainty like unclear user prompts. The paper demonstrates the effectiveness of USAM on several datasets, showing its ability to identify sources of uncertainty and improve model predictions. Overall, this paper is well-organized and theoretically grounded.

Claims And Evidence:
The main claims about uncertainty quantification in SAM are supported by clear mathematical formulation, method, proofs, and experiments. The minor concern is the claim that "the ambiguous nature of the class-agnostic foundation model SAM challenges current uncertainty quantification approaches." is not well justified. As SAM can generate ambiguous predictions (Top-K), it inherently has uncertainty awareness, making the uncertainty analysis easier. Why do the authors claim that this will challenge UQ?

Methods And Evaluation Criteria:
The proposed method introduces Bayesian Entropy Approximation in SAM, which makes sense and is technically sound. It considers uncertainty from different levels (Eq.2), which is well justified by both theoretical proofs (Sec. 3) and experiments (Sec.4.2 to Sec. 4.4).

Theoretical Claims:
I have checked the theoretical claims about the uncertainty quantification formulation (Sec. 2.2), the grounding in SAM (Sec.2.3), and Bayesian Entropy Approximation (Sec.3 and Appendix A). I did not find major theoretical errors and think that this paper is well organized.

Experimental Designs Or Analyses:
Most of the experiments were well conducted, especially for the detailed justification of claimed uncertainty terms from the model, prompt, and task aspects. The experimental analysis is also comprehensive and convincing. However, there are two major concerns. The first concern is insufficiently comparing existing UQ methods in SAM model, such as [1-3]. The second concern is the lack of comparison of specific settings focusing on uncertain predictions, like ambiguous segmentation, which is critical to highlight the strength of the proposed UQ methods [1,2].
[1] Flaws can be Applause: Unleashing Potential of Segmenting Ambiguous Objects in SAM (NeurIPS 24)
[2] Uncertainty-aware Fine-tuning of Segmentation Foundation Models (NeurIPS 24)

Supplementary Material: I have checked the mathematical proof of Bayesian entropy approximation, and more quantitative and qualitative results.

Relation To Broader Scientific Literature: The proposed method has a potentially broader impact on understanding the existing SAM model from the uncertainty perspective, thereby inspiring the algorithmic designs of the next-generation SAM.

Essential References Not Discussed: The proposed method explores the uncertainty quantification of the SAM model. However, this is not a new direction, and there are many related works. Even though the proposed method is comprehensive, technically sound, and theoretically correct, it is suggested to make necessary discussion with related UQ methods using SAM [1-2]
[1] Flaws can be Applause: Unleashing Potential of Segmenting Ambiguous Objects in SAM (NeurIPS 24)
[2] Uncertainty-aware Fine-tuning of Segmentation Foundation Models (NeurIPS 24)

Other Strengths And Weaknesses:
Strength:

    1. The paper is well organized and gives a comprehensive and theoretically sound analysis of the uncertainty in SAM.
    2. The proposed Bayesian approximation is reasonable.
    3. The perception of the model, prompt, and task uncertainty is interesting and comprehensive.
    4. The experimental justification is solid.
Weakness:
    1. Lack some comparison with related works about modelling uncertainty in SAM
    2. Lack some clarification (see Questions For Authors)

Other Comments Or Suggestions:

Questions For Authors:
    1. The authors claim that "For several tasks, quantifying the uncertainty of SAM is of particular interest.". It is suggested to clarify what tasks require measuring uncertainty in SAM.
    2. The authors are suggested to give a justification for the efficiency of the proposed method.
    3. In Sec. 4, the authors implement the method in SAM2, but Fig.1 illustrates SAM, which is inconsistent.
    4. Considering that the authors use SAM 2 as the base model, the theoretical analysis lacks a formulation for time-series signals. Will it introduce extra uncertainty when considering the object motions in videos?
    5. Lack of a comparison on the ambiguous segmentation benchmark.

Code Of Conduct: Affirmed.
Overall Recommendation: 3: Weak accept (i.e., leaning towards accept, but could also be rejected)




------> TODOs:
1. Erklären, was mit "the ambiguous nature of the class-agnostic foundation model SAM challenges current uncertainty quantification approaches"
2. Mindestens Erweiterung für Related work vorschlagen
3. Mindestens eine Methode als Competitor einbauen
4. Wie R2. Erklären, was mit SAM2 gemeint ist.
5. Ambiguous segmentation benchmark: Welche meinen die? Anschauen und vielleicht USAM drauf anwenden wenn möglich?
6. 3 Paper zitieren: "for several tasks, quantifying the uncertainty of SAM is of particular interest"
7. Efficiency: Wie bei R1



--------> REBUTTAL:

We acknowledge the in-depth review that recognizes our strengths and provides valuable directions for addressing flaws and weaknesses, particularly regarding related UQ methods in SAM. Below, we address the reviewer’s questions and concerns. Some issues are already covered in our responses to other reviewers, which we reference to reduce redundancy.

Claims and Evidence: "The ambiguous nature of the class-agnostic foundation model SAM challenges current uncertainty quantification approaches."
Thank you for pointing out that this claim in the abstract is not sufficiently elaborated in the introduction. A more detailed discussion of SAM (and other open-set segmentors) and its implications for UQ is provided in Section 2.3, "UQ in SAM."
To summarize: Most standard UQ methods, when analyzed from a general perspective, are based on MC strategies and are motivated by Bayesian principles (see Equation 1 and the following elaborations). While these methods work effectively, their theoretical justifications rely on assumptions that are often unrealistic and cannot be guaranteed in practice. For example, test-time augmentation (Wang et al., 2019), which is used to estimate aleatoric uncertainty, assumes that the sample is in-distribution and has been seen multiple times during training, with variance encoded in noisy patterns. Similarly, epistemic UQ estimators, such as model ensembles, assume that uncertain samples are out-of-distribution. These challenges, which already exist in well-established UQ approaches, are further exacerbated by the task-agnostic nature of SAM.
To the best of our knowledge, there is no general discussion in the literature on the implications and challenges of UQ in this context. However, we acknowledge that our formulation of this claim is unclear. To address this, we suggest adding a clarification before "More insights ..." (line 126, right column) as follows:

"While the presented methods work well in practice, the theoretical foundations for separating aleatoric and epistemic uncertainty remain debatable and under active discussion (Gruber et al., 2023). The task-agnostic nature of SAM further amplifies this challenge, as discussed next. More insights into ..."

Weakness 1: The issue of weak quantitative comparisons with UQ methods in SAM is closely related to the previously discussed point. As the reviewer mentioned, several papers propose UQ methods, such as [1] and [2]. However, these methods are designed for specific tasks that are not directly comparable to ours.
For example, [1] enhances variance in the latent space to sample more ambiguous segmentation outputs, while [2] estimates pixel-wise epistemic uncertainty that may arise due to domain shifts during fine-tuning. USAM neither generates multiple mask samples nor estimates pixel-wise uncertainty, making it unsuitable for both tasks.
With a generous interpretation, [1] could be integrated into our H_A calculation, or the saliency map from [2] could be used to compute entropy. However, these adaptations would not accurately reflect the original methods. 
Furthermore, our UQ comparison aligns with the state-of-the-art (SOTA) comparisons performed in [1] and [2].
In [1], UQ performance is evaluated by applying prompt perturbations to SegGPT (similar to our H_XP) and image augmentations to SEEM (similar to our H_Y). Note that the accuracy differences observed in these comparisons may be influenced by variation of the base framework. In [2], a pixel-wise equivalent to our competitor Entropy is used, termed SUM Confidence-Uncer, alongside a pixel-wise equivalent to our H_A, termed SUM Discrepancy-Uncer. These study designs underline that standard UQ methods are applicable for evaluating new UQ approaches.
Nevertheless, we acknowledge that our paper does not sufficiently address the variety of UQ approaches used in conjunction with SAM. To improve clarity, we propose using the additional page in the camera-ready version to expand Section 2.3 ("UQ in SAM") and include a discussion of more related works that propose or employ UQ with SAM, such as [1] and [2], as well as publications from the ambiguous image segmentation community.

Suggestion/Question 1: "For several tasks, quantifying the uncertainty of SAM is of particular interest". We mention some tasks in the proposed paper: For example, Vujasinovic et al. (2024) use UQ to estimate if supervision is required to correct tracking errors, or in the healthcare domain to gain trust and improve prediction (Deng et al., 2023; Zhang et al., 2023). The papers [1] and [2] mentioned by the reviewer employ UQ in SAM to sample prediction or to close the domain gap during finetuning. We will add the references to the introduction in the camera ready.

Suggestion/Question 2: A similar concern was raised by reviewer nnaG. We agree that the simplicity of our MLP does not sufficiently support claims of superior efficiency. To address this, we conducted runtime experiments demonstrating that USAM incurs minimal computational overhead and is significantly faster than MC-based methods.
For details on the experimental setup and results, please see our response to reviewer nnaG. We propose adding these findings to the camera-ready version to emphasize the efficiency of our approach.

Suggestion/Question 3 and 4 (SAM2): Our submitted paper contains ambiguities regarding our use of SAM2. For a detailed clarification, please see our response to reviewer 6x8E, where we explain these issues and propose modifications for the camera-ready versio

Suggestion/Question 5: We are uncertain how our method could be applied to the ambiguous segmentation benchmark. For instance, as stated by [X], the goal of this benchmark is to achieve "better agreement between prediction and the ground truth," measured using the Generalized Energy Distance.
In contrast, our method estimates the variance of the distribution (i.e., uncertainty). Since we do not modify SAM’s top-3 mask selection approach, our scores would be identical to those of the vanilla SAM model.
As we are not experts in the proposed benchmarks, we would appreciate any guidance on how our method could be applied and which datasets would be relevant (e.g., LIDC-IDR, B-US, MS-MRI, etc.).

[X] Rahman, Aimon, et al. "Ambiguous medical image segmentation using diffusion models." Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. 2023.

#################### R4: pXDa ########################################
Summary:

This work introduces a method for uncertainty quantification of SAM, based on Bayesian entropy formulation. A lightweight post-hoc UQ method is trained based on the formulation. Results on multiple public benchmarks demonstrate the effectiveness of the proposed method.
Claims And Evidence: Claims are clear and convincing.
Methods And Evaluation Criteria: Evaluation criteria make sense.
Theoretical Claims: Theoretical claims seem correct to me.
Experimental Designs Or Analyses: The experimental designs and analyses are reasonable to me.
Supplementary Material: I have checked the quantitative and qualitative results in the supplementary materials.
Relation To Broader Scientific Literature: This uncertainty quantification method of SAM can benefit a wide range of computer vision tasks. Considering the wide application of SAM, this method will be influential.
Essential References Not Discussed: No.
Other Strengths And Weaknesses:
Strength: 
1. The experiments on multiple public benchmarks validate the effectiveness of the proposed method comprehensively.
Other Comments Or Suggestions: N/A.
Questions For Authors: N/A.
Code Of Conduct: Affirmed.
Overall Recommendation: 3: Weak accept (i.e., leaning towards accept, but could also be rejected)



-----> TODOs: Macht so absolut gar keinen Punkt auf. Nett für das Review bedanken und nochmal drauf fragen, wie das Paper verbessert werden könnten?

-----> REBUTTAL:

We thank the reviewer for the feedback and positive assessment. To further support the reviewer’s inclination toward acceptance, we would like to highlight the linked code repository in the main paper, which demonstrates the ease of use of our proposed framework. We remain open to any additional questions, remarks, or suggestions to refine our proposed paper during the author-reviewer discussion.



#################### Confidential Comment to AC ########################################

Dear Area Chair,

First of all, we are glad that most reviewers submitted valuable reviews that helped us to remove ambiguities and strengthen the paper. However, we are concerned about the missing feedback, especially from Reviewer nnaG, who is leaning towards rejection due to concerns that we addressed during our rebuttal.

We disagree with Weakness 1, which states that we do not compare to SAM-specific UQ. While the direct use of application-specific SAM-UQ papers is not suitable, we compare our method to the most commonly used UQ techniques employed in works that build on SAM, as we elaborated in more detail in the rebuttal to Reviewer 3EoJ. The mentioned Weakness 2, regarding insufficiently elaborated MLP design choices, is due to the fact that we use the default SAM MLP — something we can and will clarify in a single sentence in the camera-ready version. The reviewer’s final Weakness 3 actually turns out to be a strength after conducting the requested experiments. As we showed in the rebuttal, runtime experiments demonstrate that our method is the most efficient among the compared approaches.

Because the first concern is debatable and the others can be directly resolved — and even improve the paper with just a few lines of clarification in the camera-ready version — we are worried about the apparent lack of engagement with our rebuttal.

Given this lack of response to our clarification of all concerns, we kindly request that you take our rebuttal into account when weighing Reviewer nnaG's assessment in your decision-making process.

Kind regards,
The authors
